Hazelnut: A Bidirectionally Typed Structure Editor Calculus

Structure editors allow programmers to edit the tree structure of a program directly. This can have cognitive benefits, particularly for novice and end-user programmers. It also simplifies matters for tool designers, because they do not need to contend with malformed program text. This paper defines Hazelnut, a structure editor based on a small bidirectionally typed lambda calculus extended with holes and a cursor. Hazelnut goes one step beyond syntactic well-formedness: its edit actions operate over statically meaningful incomplete terms. Naively, this would force the programmer to construct terms in a rigid "outside-in" manner. To avoid this problem, the action semantics automatically places terms assigned a type that is inconsistent with the expected type inside a hole. This safely defers the type consistency check until the term inside the hole is finished. Hazelnut is a foundational type-theoretic account of typed structure editing, rather than an end-user tool itself. To that end, we describe how Hazelnut's rich metatheory, which we have mechanized in Agda, guides the definition of an extension to the calculus. We also discuss various plausible evaluation strategies for terms with holes, and in so doing reveal connections with gradual typing and contextual modal type theory, the Curry-Howard interpretation of contextual modal logic. Finally, we discuss how Hazelnut's semantics lends itself to implementation as a functional reactive program. Our reference implementation is written using js_of_ocaml.

==> dynamics.tex <==
%% Cyrus: We took a look at the dynamics. Overall it seems like the
%% right idea. We noticed:

%% Done: 1) The stepping rules are non-deterministic (i.e. you can
%% step the right or left of e1 + e2 in any order). Might be useful to
%% make them deterministic.

%% Done (mostly): 2) The premises that have disjunctions in them could
%% be broken out into two rules -- this would take a little more space
%% but follows the usual conventions more closely.

%% Done (mostly): 3) We need to add the ``ceil'' forms to the grammar
%% of \dot{e} (you just used e) and give them a static semantics.

%% TODO: 4) We need to figure out (the analogs of) canonical forms,
%% preservation and progress -- I guess we had decided on defining a
%% declarative statics to do that. Ian has started to prove the
%% correspondence (sans the ceil forms).

%% #4 seems like the most important next step.

\begin{figure}[htbp]
  \centering

  \judgbox{\hexp~\textsf{value}}{H-Expression $\hexp$ is a closed value}
  \begin{mathpar}
    \Infer{V-num}
          { }
          {\hnum{n}~\textsf{value}}
    \and
    \Infer{V-lam}
        {}
        {\hlam{x}{\hexp}~\textsf{value}}
  \end{mathpar}
  
  \caption{Value forms}
  \label{fig:judg-value}
\end{figure}

\begin{figure}[htbp]
  \centering

  \judgbox{\hexp~\textsf{final}}{H-Expression $\hexp$ is final}
  \begin{mathpar}
    \Infer{F-val}
          {\hexp~\textsf{value}}
          {\hexp~\textsf{final}}
    \and
    \Infer{F-filled}
          {\hexp~\textsf{final}}
          {\hhole{\hexp}~\textsf{final}}
    \and
    \Infer{F-unfilled}
          { }
          {\hhole{}~\textsf{final}}
    \and
    \Infer{F-indet}
        {\hexp~\textsf{indet}}
        {\hindet{\hexp}~\textsf{final}}
  \end{mathpar}
  
  \caption{Final forms}
  \label{fig:judg-value}
\end{figure}

\begin{figure}[htbp]
  \centering

  \judgbox{\hexp~\textsf{indet}}{H-Expression~$\hexp$ is indeterminate}
  \begin{mathpar}
    \Infer{I-plus$_1$}
          { \hexp_1~\textsf{final} \\
            \hexp_2~\textsf{final} \\
            \hexp_1 \ne \hnum{n_1}
          }
          {\hadd{e_1}{e_2}~\textsf{indet}}
    \and
    \Infer{I-plus$_2$}
          { \hexp_1~\textsf{final} \\
            \hexp_2~\textsf{final} \\
            \hexp_2 \ne \hnum{n_2}
          }
          {\hadd{\hexp_1}{\hexp_2}~\textsf{indet}}
    \and
    \Infer{I-app}
          { \hexp_1~\textsf{final} \\
            \hexp_2~\textsf{final} \\
            \hexp_1 \ne \hlam{x}{\hexp_1'}
          }
          {\hap{\hexp_1}{\hexp_2}~\textsf{indet}}
    \and
  \end{mathpar}
  
  \caption{Indeterminate forms}
  \label{fig:judg-value}
\end{figure}

\begin{figure}[htbp]
  \centering

  \judgbox{\hexp_1 \longrightarrow \hexp_2}{H-Expression $\hexp_1$ steps to~$\hexp_2$}
  \begin{mathpar}
    \Infer{S-plus$_1$}
          { \hexp_1 \longrightarrow \hexp_1' }
          { \hadd{\hexp_1}{\hexp_2} \longrightarrow \hadd{\hexp_1'}{\hexp_2} }

    \Infer{S-plus$_2$}
          { \hexp_1~\textsf{final}
            \\
            \hexp_2 \longrightarrow \hexp_2' }
          { \hadd{\hexp_1}{\hexp_2} \longrightarrow \hadd{\hexp_1}{\hexp_2'} }

    \Infer{S-plus$_3$}
          { n_1 + n_2 = n_3 }
          { \hadd{\hnum{n_1}}{\hnum{n_2}} \longrightarrow \hnum{n_3} }

   \Infer{S-plus$_4$}
          { \hexp_1~\textsf{final} ~~ ~~ ~~
            \hexp_2~\textsf{final} 
            \\\\
            \left(\hexp_1 \ne \hnum{n_1} \vee \hexp_2 \ne \hnum{n_2}\right)
          }
          { \hadd{\hexp_1}{\hexp_2} \longrightarrow \hindet{\hadd{\hexp_1}{\hexp_2}} }

    \Infer{S-ap$_1$}
          { \hexp_1 \longrightarrow \hexp_1' }
          { \hap{\hexp_1}{\hexp_2} \longrightarrow \hap{\hexp_1'}{\hexp_2} }

    \Infer{S-ap$_2$}
          { \hexp_2 \longrightarrow \hexp_2'
            \\
            \hexp_1~\textsf{final}
          }
          { \hap{\hexp_1}{\hexp_2} \longrightarrow \hap{\hexp_1}{\hexp_2'} }

    \Infer{S-ap$_3$}
          { \hexp_2~\textsf{final} }
          { \hap{\hlam{x}{\hexp_1}}{\hexp_2} \longrightarrow [\hexp_2/x]\hexp_1 }

   \Infer{S-ap$_4$}
          { \hexp_1~\textsf{final} ~~ ~~ ~~
            \hexp_2~\textsf{final}
            \\\\
            \hexp_1 \ne \hlam{x}{\hexp_1'} ~~ ~~ ~~ ~~ ~~ ~~ ~~ { }
          }
          { \hap{\hexp_1}{\hexp_2} \longrightarrow \hindet{\hap{\hexp_1}{\hexp_2}} }

  \end{mathpar}
  
  \caption{Small-step operational semantics.}
  \label{fig:judg-value}
\end{figure}

% Q: Are we running programs with ascriptions?
% No. We erase the ascriptions before running. Ascriptions below are
%
% Q: Are the ascriptions needed to type-check the programs?
% No. The ascriptions are needed to check the programs algorithmically, not to derive typing derivations.
% (Q: How do ascriptions, holes, and typing derivations interact?)
%
% Q: Does it ever make sense to run open programs? (i.e., run programs with ``free variables''?)
%  -- Yes, but only in the sense that we can bind holes to variables,
%     ascribe them types, and (attempt to) compute with them.
%
% Example: (where '?' means "empty hole")
%  let x = ? : int -> int in
%  let y = ? : int in
%  x y : int
% ==erase==>
%  let x = ? in
%  let y = ? in
%  x y
% -->
%  let y = ? in
%  ? y
% -->
%  ? ?
% --> 
%  (indet ? ?)

We extend the syntax of H-Expressions as follows:
\[
\hexp ::= \cdots~|~\hindet{\hexp}
\]

Here are some things that we want to prove:

\textbf{Def}~(Ascription erasure). 
\\
$\herase{\hexp}$ is the same as $\hexp$, but without its type ascriptions.
%
All cases are congruences, except for the ascription case, where $\herase{\hexp : \htau} = \hexp$.

\textbf{Def}~(Declarative typing).
\\
The judgement $\hGamma \vdash \hexp : \htau$ is a type assignment
system for erased terms.  It is declarative, and unlike the
bidirectional rules, is not algorithmic.
%
We employ it to relate bidirectionally-typed terms to (erased) terms
that enjoy type soundness with respect to the dynamics.

\textbf{Conjecture}~(Bidirectional implies declarative).
\\
(i) If $\hsyn{\hGamma}{\hexp}{\htau}$ then $\hGamma \vdash \herase{\hexp} : \htau$.
\\
(ii) If $\hana{\hGamma}{\hexp}{\htau}$ then $\hGamma \vdash \herase{\hexp} : \htau$.

\textbf{Conjecture}~(Substitution).
\\
If $\hGamma, x : \tau_x \vdash \hexp : \htau$
\\
and $\hexp'~\textsf{final}$~~~(do we actually need this condition?)
\\
and $\hGamma \vdash \hexp' : \htau_x$
\\
then $\hGamma \vdash \hexp[\hexp' / x] : \htau$

% Q: Do we need to enforce that hexp' is final?

\textbf{Conjecture}~(Canonical forms)
\\
If $\cdot \vdash \hexp : \htau$
\\
and $\hexp~\textsf{final}$ then
\begin{itemize}
\item if $\hexp = \hindet{\hexp'}$ then $\hexp'~\textsf{indet}$ and $\cdot \vdash \hexp' : \htau$
%\marginnote{Since $\hexp'~\textsf{indet}$, the conjecture applies to $\hexp'$.}
\item else:
\begin{itemize}
\item if $\htau = \tnum$ then exists $\hnum{n}$ such that $\hexp = \hnum{n}$.
\item else if $\htau = \tarr{\htau_1}{\htau_2}$ then exists $x$ and $\hexp'$ such that $\hexp = \hlam{x}{\hexp'}$
\item else if $\htau = \tehole$ then either:
\begin{itemize}
\item $\hexp = \hehole$, or
\item exists $\htau'$ and $\hexp'$ such that $\hexp = \hhole{\hexp'}$, $\hexp'~\textsf{final}$ and $\cdot \vdash \hexp' : \htau'$
\end{itemize}
\end{itemize}
\end{itemize}

\textbf{Conjecture}~(Progresss).
\\
If $\cdot \vdash \hexp_1 : \htau$
\\
then either $\hexp_1~\textsf{final}$
\\
or exists $\hexp_2$ such that $\hexp_1 \longrightarrow \hexp_2$.

\textbf{Conjecture}~(Preservation).
\\
If $\cdot\vdash \hexp_1 : \htau$ 
\\
and $\hexp_1 \longrightarrow \hexp_2$
\\
then $\cdot \vdash \hexp_2 : \htau$

